Learning Topological Representations for Deep Image Understanding

In many scenarios, especially biomedical applications, the correct delineation of complex fine-scaled structures such as neurons, tissues, and vessels is critical for downstream analysis. Despite the strong predictive power of deep learning methods, they do not provide a satisfactory representation of these structures, thus creating significant barriers in scalable annotation and downstream analysis. In this dissertation, we tackle such challenges by proposing novel representations of these topological structures in a deep learning framework. We leverage the mathematical tools from topological data analysis, i.e., persistent homology and discrete Morse theory, to develop principled methods for better segmentation and uncertainty estimation, which will become powerful tools for scalable annotation.

==> title.tex <==
%
% File: Title.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the title page
%
% UoB guidelines:
% 
% At the top of the title page, within the margins, the dissertation should give the title and, if 
% necessary, sub-title and volume number. If the dissertation is in a language other than English, the 
% title must be given in that language and in English. The full name of the author should be in the 
% centre of the page. At the bottom centre should be the words ?A dissertation submitted to the 
% University of Bristol in accordance with the requirements for award of the degree of ? in the 
% Faculty of ...?, with the name of the school and month and year of submission. The word count of 
% the dissertation (text only) should be entered at the bottom right-hand side of the page.
%
%

%\begin{titlingpage}
%\begin{SingleSpace}
%\calccentering{\unitlength} 
%\begin{adjustwidth*}{\unitlength}{-\unitlength}
%\vspace*{1mm}
\begin{center}
\rule[0.5ex]{\linewidth}{2pt}\vspace*{-\baselineskip}\vspace*{3.2pt}
\rule[0.5ex]{\linewidth}{1pt}\\[\baselineskip]
{\huge Automated Segmentation of Anatomies in CT scans using Deep Learning Techniques}\\[4mm]
%{\Large \textit{Subtitle}}\\
\rule[0.5ex]{\linewidth}{1pt}\vspace*{-\baselineskip}\vspace{3.2pt}
\rule[0.5ex]{\linewidth}{2pt}\\
\vspace{5mm}
{A Dissertation presented\\}
{by}\\
\vspace{5mm}
{\large\textsc{Praitayini Knaakaraj\\ }} %\\mnroy@cs.stonybrook.edu}\\
%{mnroy@cs.stonybrook.edu \\}
{ to}\\
\vspace{5mm}
{{The Graduate School in Partial Fulfillment of the Requirements for the Degree of\\ }} %\\mnroy@cs.stonybrook.edu}\\
\vspace{3mm}
{\large\textsc{Master of Science }\\}
{in}\\
{\large\textsc {Department of Biomedical Informatics}}\\
\textsc{Stony Brook University}\\
\vspace{3mm}
\vspace{5mm}
%\begin{figure}[H]
%\centering
  \includegraphics[height=3.5cm, width=4.5cm]{figures/stonybrook.jpg}\\
%\end{figure}

%\vspace{6mm}
%{\large Department of Computer Science\\
%\textsc{Stony Brook University}}\\
%\vspace{11mm}
%\begin{minipage}{10cm}

%\end{minipage}\\
%\vspace{9mm}
{\medium \textsc{May 3, 2019}}
\vspace{5mm}

%\centering
\begin{tabular}{c c c}

\textbf{Adviser} & \textbf{Committee} & \textbf{Committee} \\
Fusheng Wang & Janos G. Hajagos & Jinkoo Kim \\
Associate Professor & Research Assistant Professor & Medical Physicists \\
Department of  & Department of & Radiation Oncology  \\
Biomedical Informatics & Biomedical Informatics & 
%Rad
\end{tabular}


\end{center}
%\begin{flushright}
%{\small Word count: ten thousand and four}
%\end{flushright}
%\end{adjustwidth*}
%\end{SingleSpace}
%\end{titlingpage}

